An Eulerian-Lagrangian discontinuous Galerkin method for transport problems and its application to nonlinear dynamics

We propose a new Eulerian-Lagrangian (EL) discontinuous Galerkin (DG) method. The method is designed as a generalization of the semi-Lagrangian (SL) DG method for linear advection problems proposed in [J. Sci. Comput. 73: 514-542, 2017], which is formulated based on an adjoint problem and tracing upstream cells by tracking characteristics curves highly accurately. In the SLDG method, depending on the velocity field, upstream cells could be of arbitrary shape. Thus, a more sophisticated approximation to sides of the upstream cells is required to get high order approximation. For example, quadratic-curved (QC) quadrilaterals were proposed to approximate upstream cells for a third-order spatial accuracy in a swirling deformation example. In this paper, for linear advection problems, we propose a more general formulation, named the ELDG method. The scheme is formulated based on a {\em modified} adjoint problem for which the upstream cells are always quadrilaterals, which avoids the need to use QC quadrilaterals in the SLDG algorithm. The newly proposed ELDG method can be viewed as a new general framework, in which both the classical Eulerian Runge-Kutta DG formulation and the SL DG formulation can fit in. Numerical results on linear transport problems, as well as the nonlinear Vlasov and incompressible Euler dynamics using the exponential RK time integrators, are presented to demonstrate the effectiveness of the ELDG method.

==> schematic_eldg1d_st2.tex <==
\begin{figure}[h!]
\centering
\subfigure[]{
\begin{tikzpicture}[x=1cm,y=1cm]%[scale=1.0]
  \begin{scope}[thick]


   \draw (-3,3) node[fill=white] {};
    \draw (-3,-1) node[fill=white] {};
    \draw[black]                   (-3,0) node[left] {} -- (3,0)
                                        node[right]{$t^{n}$};
    \draw[black] (-3,2) node[left] {$$} -- (3,2)
                                        node[right]{$t^{n+1}$};
     \draw[snake=ticks,segment length=2.4cm] (-2.4,2) -- (0,2) node[above left] {$x_{j-\frac12}$};
     \draw[snake=ticks,segment length=2.4cm] (0,2) -- (2.4,2) node[above right] {$x_{j+\frac12}$};

          \draw[snake=ticks,segment length=2.4cm] (-2.4,0) -- (0,0);
     \draw[snake=ticks,segment length=2.4cm] (0,0) -- (2.4,0);
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
            \draw[-latex,dashed,red] (0.,2) node[left] {$$} to[out=240,in=85] (-1.5+0.7,0)
                                        node[black,below]{$x_{j-\frac12}^\star$ };

                \draw[-latex,dashed,red] (2.4,2) node[left] {$$} to[out=245,in=85] (1.6+0.4,0)
                                        node[black,below right]{ $x_{j+\frac12}^\star$};
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


  %\node[blue, rotate=0] (a) at ( 0.7  ,1.3)  { \tiny $ \frac{d\tilde{x}(t ) }{dt}= a(\tilde{x}(t ),t)$, };
  %\node[blue, rotate=0] (a) at ( 0.7  ,1.3-0.5)  {\tiny   $\tilde{x}(t^{n+1} )={x_{j+\frac12}}$ };

  \node[  rotate=0] (a) at ( 0.6  ,1.3)  { \scriptsize Characteristics tracing };

  \draw[-latex  ](  1.7, 1.1 )node[right=-3pt,scale=1.0]{ }
        to[out=320,in=150] ( 2.1  , 0.8) node[below=2pt] { };

  %{\tiny $\left.\frac{d\tilde{x}(t;x,t^{n+1}) }{dt}= a(\tilde{x}(t;x,t^{n+1}),t)\right|_{x_{j-\frac12}}$ };
  %\node[blue, rotate=0] (a) at (3,1.) {\tiny $\frac{d\tilde{x}(t;x_{j+\frac12},t^{n+1})}{dt}= a(\tilde{x}(t;x_{j+\frac12},t^{n+1}),t)$ };
  \end{scope}
\end{tikzpicture}
 }
 \subfigure[]{
\begin{tikzpicture}[x=1cm,y=1cm]%[scale=1.0]
  \begin{scope}[thick]


 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%            \draw[-latex,dashed,red] (0.,2) node[left] {$$} to[out=240,in=85] (-1.5+0.7,0)
%                                        node[black,below]{  };
%
%                \draw[-latex,dashed,red] (2.4,2) node[left] {$$} to[out=245,in=85] (1.6+0.4,0)
%                                        node[black,below right]{ };
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


    \draw[white,fill=blue!4] (0,2) -- (-0.8,0)  -- (2,0) -- (2.4, 2)
      -- cycle;
    \node[blue!80, rotate=0] (a) at ( 1. ,1.5 ) {\Large $\Omega_{j}$ };




   \draw (-3,3) node[fill=white] {};
    \draw (-3,-1) node[fill=white] {};
    \draw[black]                   (-3,0) node[left] {} -- (3,0)
                                        node[right]{$t^{n}$};
    \draw[black] (-3,2) node[left] {$$} -- (3,2)
                                        node[right]{$t^{n+1}$};
     \draw[snake=ticks,segment length=2.4cm] (-2.4,2) -- (0,2) node[above left] {$x_{j-\frac12}$};
     \draw[snake=ticks,segment length=2.4cm] (0,2) -- (2.4,2) node[above right] {$x_{j+\frac12}$};

          \draw[snake=ticks,segment length=2.4cm] (-2.4,0) -- (0,0);
     \draw[snake=ticks,segment length=2.4cm] (0,0) -- (2.4,0);
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%            \draw[-latex,dashed,blue] (0.,2) node[left] {$$} to[out=240,in=85] (-1.5+0.7,0)
%                                        node[black,below]{$x_{j-\frac12}^\star$ };
%
%                \draw[-latex,dashed,blue] (2.4,2) node[left] {$$} to[out=245,in=85] (1.6+0.4,0)
%                                        node[black,below right]{ $x_{j+\frac12}^\star$};


  \draw[-latex, blue] (0.,2) node[left] {$$} -- (-1.5+0.7,0)  node[black,below]{$x_{j-\frac12}^\star$ };

  \draw[-latex, blue] (2.4,2) node[left] {$$} -- (1.6+0.4,0)  node[black,below right]{ $x_{j+\frac12}^\star$};



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

  \draw[-latex,blue!50,dashed] (0.6,2) node[left] {$$} -- (-0.8+0.25*2.8 ,0)
                                        node[black,below]{ };
  \draw[-latex,blue!50,dashed] (1.2,2) node[left] {$$} -- (-0.8+0.5*2.8 ,0)
                                        node[black,below]{ };
  \draw[-latex,blue!50,dashed] (1.8,2) node[left] {$$} -- (-0.8+0.75*2.8 ,0)
                                        node[black,below]{ };

%%%%%%%%%%%%%%%%
\draw[-latex,thick,blue](0.4,1)node[right,scale=1.]{\footnotesize $\tilde{I}_j(t)$}
        to[out=180,in=0] (-0.4,1) node[above left=2pt] {$$};  %%%thick ʵ�ߣ� dashed ����

\draw[-latex,thick,blue](1.3,1)node[right,scale=1.]{ }
        to[out=0,in=180] (2.2,1) node[above left=2pt] {$$};  %%%thick ʵ�ߣ� dashed ����





  \node[blue, rotate=67] (a) at (-0.7 ,1.) { $\nu_{j-\frac12}$ };
  \node[blue, rotate=80] (a) at (2.5,1.) { $\nu_{j+\frac12}$ };


  \end{scope}
\end{tikzpicture}
 }
\caption{Illustration for the  space-time region of the alternative ELDG formulation. %\QQ{Merge two figures into one}
 }
\label{st2}
\end{figure}

